Self-Distilled Representation Learning for Time Series

Self-supervised learning for time-series data holds potential similar to that recently unleashed in Natural Language Processing and Computer Vision. While most existing works in this area focus on contrastive learning, we propose a conceptually simple yet powerful non-contrastive approach, based on the data2vec self-distillation framework. The core of our method is a student-teacher scheme that predicts the latent representation of an input time series from masked views of the same time series. This strategy avoids strong modality-specific assumptions and biases typically introduced by the design of contrastive sample pairs. We demonstrate the competitiveness of our approach for classification and forecasting as downstream tasks, comparing with state-of-the-art self-supervised learning methods on the UCR and UEA archives as well as the ETT and Electricity datasets.

==> figures/architecture.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Path Data [id:dp577693984949704] 
\draw   (84.53,35.18) -- (84.53,47.75) .. controls (84.53,50.07) and (83.53,51.94) .. (82.3,51.94) -- (13.01,51.94) .. controls (11.78,51.94) and (10.78,50.07) .. (10.78,47.75) -- (10.78,35.18) .. controls (10.78,32.87) and (11.78,30.99) .. (13.01,30.99) -- (82.3,30.99) .. controls (83.53,30.99) and (84.53,32.87) .. (84.53,35.18) -- cycle (84,64.25) -- (84,76.82) .. controls (84,79.13) and (83,81.01) .. (81.77,81.01) -- (12.48,81.01) .. controls (11.24,81.01) and (10.25,79.13) .. (10.25,76.82) -- (10.25,64.25) .. controls (10.25,61.94) and (11.24,60.06) .. (12.48,60.06) -- (81.77,60.06) .. controls (83,60.06) and (84,61.94) .. (84,64.25) -- cycle (84,123.01) -- (84,135.57) .. controls (84,137.89) and (83,139.76) .. (81.77,139.76) -- (12.48,139.76) .. controls (11.24,139.76) and (10.25,137.89) .. (10.25,135.57) -- (10.25,123.01) .. controls (10.25,120.69) and (11.24,118.82) .. (12.48,118.82) -- (81.77,118.82) .. controls (83,118.82) and (84,120.69) .. (84,123.01) -- cycle (84,213.3) -- (84,225.87) .. controls (84,228.18) and (83,230.06) .. (81.77,230.06) -- (12.48,230.06) .. controls (11.24,230.06) and (10.25,228.18) .. (10.25,225.87) -- (10.25,213.3) .. controls (10.25,210.99) and (11.24,209.11) .. (12.48,209.11) -- (81.77,209.11) .. controls (83,209.11) and (84,210.99) .. (84,213.3) -- cycle (84,93.94) -- (84,106.51) .. controls (84,108.82) and (83,110.69) .. (81.77,110.69) -- (12.48,110.69) .. controls (11.24,110.69) and (10.25,108.82) .. (10.25,106.51) -- (10.25,93.94) .. controls (10.25,91.62) and (11.24,89.75) .. (12.48,89.75) -- (81.77,89.75) .. controls (83,89.75) and (84,91.62) .. (84,93.94) -- cycle (84,182.38) -- (84,194.95) .. controls (84,197.26) and (83,199.14) .. (81.77,199.14) -- (12.48,199.14) .. controls (11.24,199.14) and (10.25,197.26) .. (10.25,194.95) -- (10.25,182.38) .. controls (10.25,180.06) and (11.24,178.19) .. (12.48,178.19) -- (81.77,178.19) .. controls (83,178.19) and (84,180.06) .. (84,182.38) -- cycle (84.25,152.07) -- (84.25,164.64) .. controls (84.25,166.96) and (83.25,168.83) .. (82.02,168.83) -- (12.23,168.83) .. controls (11,168.83) and (10,166.96) .. (10,164.64) -- (10,152.07) .. controls (10,149.76) and (11,147.88) .. (12.23,147.88) -- (82.02,147.88) .. controls (83.25,147.88) and (84.25,149.76) .. (84.25,152.07) -- cycle ;
%Rounded Rect [id:dp807994405776387] 
\draw   (122,82.6) .. controls (122,65.15) and (136.15,51) .. (153.6,51) -- (489.6,51) .. controls (507.05,51) and (521.2,65.15) .. (521.2,82.6) -- (521.2,177.4) .. controls (521.2,194.85) and (507.05,209) .. (489.6,209) -- (153.6,209) .. controls (136.15,209) and (122,194.85) .. (122,177.4) -- cycle ;
%Right Arrow [id:dp2762111553721591] 
\draw   (92,122.92) -- (102,122.92) -- (102,117.67) -- (112,128.17) -- (102,138.67) -- (102,133.42) -- (92,133.42) -- cycle ;
%Rounded Rect [id:dp4672766923655107] 
\draw   (130,101.84) .. controls (130,100.49) and (131.09,99.4) .. (132.44,99.4) -- (139.76,99.4) .. controls (141.11,99.4) and (142.2,100.49) .. (142.2,101.84) -- (142.2,154.96) .. controls (142.2,156.31) and (141.11,157.4) .. (139.76,157.4) -- (132.44,157.4) .. controls (131.09,157.4) and (130,156.31) .. (130,154.96) -- cycle ;
%Rounded Rect [id:dp3694998546218755] 
\draw   (154,103.64) .. controls (154,101.3) and (155.9,99.4) .. (158.24,99.4) -- (170.96,99.4) .. controls (173.3,99.4) and (175.2,101.3) .. (175.2,103.64) -- (175.2,154.16) .. controls (175.2,156.5) and (173.3,158.4) .. (170.96,158.4) -- (158.24,158.4) .. controls (155.9,158.4) and (154,156.5) .. (154,154.16) -- cycle ;
%Rounded Rect [id:dp35419254919670573] 
\draw   (226,106.44) .. controls (226,102) and (229.6,98.4) .. (234.04,98.4) -- (258.16,98.4) .. controls (262.6,98.4) and (266.2,102) .. (266.2,106.44) -- (266.2,150.36) .. controls (266.2,154.8) and (262.6,158.4) .. (258.16,158.4) -- (234.04,158.4) .. controls (229.6,158.4) and (226,154.8) .. (226,150.36) -- cycle ;
%Rounded Rect [id:dp8443759512498554] 
\draw   (283,109.4) .. controls (283,102.77) and (288.37,97.4) .. (295,97.4) -- (331.2,97.4) .. controls (337.83,97.4) and (343.2,102.77) .. (343.2,109.4) -- (343.2,145.4) .. controls (343.2,152.03) and (337.83,157.4) .. (331.2,157.4) -- (295,157.4) .. controls (288.37,157.4) and (283,152.03) .. (283,145.4) -- cycle ;
%Rounded Rect [id:dp8673258258714367] 
\draw   (429.33,109.73) .. controls (429.33,103.11) and (434.71,97.73) .. (441.33,97.73) -- (477.53,97.73) .. controls (484.16,97.73) and (489.53,103.11) .. (489.53,109.73) -- (489.53,145.73) .. controls (489.53,152.36) and (484.16,157.73) .. (477.53,157.73) -- (441.33,157.73) .. controls (434.71,157.73) and (429.33,152.36) .. (429.33,145.73) -- cycle ;
%Straight Lines [id:da2681563210316158] 
\draw    (142,128.17) -- (154.33,128.17) ;
%Straight Lines [id:da10619932483558947] 
\draw    (175.33,128.17) -- (187,128.17) ;
%Straight Lines [id:da7297009105232599] 
\draw    (214.33,128.17) -- (226,128.17) ;
%Straight Lines [id:da2942726512982272] 
\draw    (266.33,128.17) -- (283.33,128.17) ;
%Straight Lines [id:da6504412103021651] 
\draw    (343.33,128.17) -- (356.33,128.17) ;
%Straight Lines [id:da8427548680494807] 
\draw    (416.33,127.83) -- (429.33,127.83) ;
%Curve Lines [id:da14304439240947064] 
\draw    (147,127.83) .. controls (147,59.83) and (181.33,60.83) .. (181.67,127.83) ;
%Curve Lines [id:da8940665832518804] 
\draw    (220.33,128.17) .. controls (220.33,60.17) and (273.33,60.83) .. (273.67,127.83) ;
%Curve Lines [id:da8280629010488143] 
\draw    (273.67,127.83) .. controls (273.67,59.83) and (350,60.83) .. (350.33,127.83) ;
%Curve Lines [id:da7615027380737611] 
\draw    (422.67,127.83) .. controls (422.67,59.83) and (500,60.83) .. (500.33,127.83) ;
%Straight Lines [id:da5145067659841966] 
\draw    (489.67,127.17) -- (560.67,127.33) ;
\draw [shift={(563.67,127.33)}, rotate = 180.13] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
%Straight Lines [id:da6673000955841928] 
\draw    (117,128.17) -- (130,128.17) ;
%Shape: Path Data [id:dp08631101226447457] 
\draw   (638.53,33.52) -- (638.53,46.08) .. controls (638.53,48.4) and (637.53,50.27) .. (636.3,50.27) -- (567.01,50.27) .. controls (565.78,50.27) and (564.78,48.4) .. (564.78,46.08) -- (564.78,33.52) .. controls (564.78,31.2) and (565.78,29.33) .. (567.01,29.33) -- (636.3,29.33) .. controls (637.53,29.33) and (638.53,31.2) .. (638.53,33.52) -- cycle (638,62.58) -- (638,75.15) .. controls (638,77.47) and (637,79.34) .. (635.77,79.34) -- (566.48,79.34) .. controls (565.24,79.34) and (564.25,77.47) .. (564.25,75.15) -- (564.25,62.58) .. controls (564.25,60.27) and (565.24,58.4) .. (566.48,58.4) -- (635.77,58.4) .. controls (637,58.4) and (638,60.27) .. (638,62.58) -- cycle (638,121.34) -- (638,133.91) .. controls (638,136.22) and (637,138.1) .. (635.77,138.1) -- (566.48,138.1) .. controls (565.24,138.1) and (564.25,136.22) .. (564.25,133.91) -- (564.25,121.34) .. controls (564.25,119.03) and (565.24,117.15) .. (566.48,117.15) -- (635.77,117.15) .. controls (637,117.15) and (638,119.03) .. (638,121.34) -- cycle (638,211.63) -- (638,224.2) .. controls (638,226.52) and (637,228.39) .. (635.77,228.39) -- (566.48,228.39) .. controls (565.24,228.39) and (564.25,226.52) .. (564.25,224.2) -- (564.25,211.63) .. controls (564.25,209.32) and (565.24,207.45) .. (566.48,207.45) -- (635.77,207.45) .. controls (637,207.45) and (638,209.32) .. (638,211.63) -- cycle (638,92.27) -- (638,104.84) .. controls (638,107.15) and (637,109.03) .. (635.77,109.03) -- (566.48,109.03) .. controls (565.24,109.03) and (564.25,107.15) .. (564.25,104.84) -- (564.25,92.27) .. controls (564.25,89.96) and (565.24,88.08) .. (566.48,88.08) -- (635.77,88.08) .. controls (637,88.08) and (638,89.96) .. (638,92.27) -- cycle (638,180.71) -- (638,193.28) .. controls (638,195.59) and (637,197.47) .. (635.77,197.47) -- (566.48,197.47) .. controls (565.24,197.47) and (564.25,195.59) .. (564.25,193.28) -- (564.25,180.71) .. controls (564.25,178.4) and (565.24,176.52) .. (566.48,176.52) -- (635.77,176.52) .. controls (637,176.52) and (638,178.4) .. (638,180.71) -- cycle (638.25,150.41) -- (638.25,162.97) .. controls (638.25,165.29) and (637.25,167.16) .. (636.02,167.16) -- (566.23,167.16) .. controls (565,167.16) and (564,165.29) .. (564,162.97) -- (564,150.41) .. controls (564,148.09) and (565,146.22) .. (566.23,146.22) -- (636.02,146.22) .. controls (637.25,146.22) and (638.25,148.09) .. (638.25,150.41) -- cycle ;
%Rounded Rect [id:dp4491604334619148] 
\draw  [color={rgb, 255:red, 249; green, 249; blue, 249 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 171; blue, 5 }  ,fill opacity=0.31 ] (123.67,87.28) .. controls (123.67,71.54) and (136.43,58.77) .. (152.17,58.77) -- (245.16,58.77) .. controls (260.9,58.77) and (273.67,71.54) .. (273.67,87.28) -- (273.67,172.8) .. controls (273.67,188.54) and (260.9,201.31) .. (245.16,201.31) -- (152.17,201.31) .. controls (136.43,201.31) and (123.67,188.54) .. (123.67,172.8) -- cycle ;
%Rounded Rect [id:dp8460552377863944] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 19; green, 154; blue, 251 }  ,fill opacity=0.26 ] (273.67,89.2) .. controls (273.67,73.81) and (286.14,61.33) .. (301.53,61.33) -- (482.47,61.33) .. controls (497.86,61.33) and (510.33,73.81) .. (510.33,89.2) -- (510.33,172.8) .. controls (510.33,188.19) and (497.86,200.67) .. (482.47,200.67) -- (301.53,200.67) .. controls (286.14,200.67) and (273.67,188.19) .. (273.67,172.8) -- cycle ;

% Text Node
\draw (65,32.4) node [anchor=north west][inner sep=0.75pt]    {$x_{1}$};
% Text Node
\draw (65,59.4) node [anchor=north west][inner sep=0.75pt]    {$x_{2}$};
% Text Node
\draw (66,210.4) node [anchor=north west][inner sep=0.75pt]    {$x_{t}$};
% Text Node
\draw (31,246.4) node [anchor=north west][inner sep=0.75pt]    {$R^{DxT}$};
% Text Node
\draw (361,170.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {average};
% Text Node
\draw (619,30.73) node [anchor=north west][inner sep=0.75pt]    {$h_{1}$};
% Text Node
\draw (618.33,57.73) node [anchor=north west][inner sep=0.75pt]    {$h_{2}$};
% Text Node
\draw (620,208.73) node [anchor=north west][inner sep=0.75pt]    {$h_{t}$};
% Text Node
\draw (585,244.73) node [anchor=north west][inner sep=0.75pt]    {$R^{HxT}$};
% Text Node
\draw (373.33,117.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% Text Node
\draw (192,115.33) node [anchor=north west][inner sep=0.75pt]   [align=left] {...};
% Text Node
\draw (171,171.67) node [anchor=north west][inner sep=0.75pt]   [align=left] {backbone};


\end{tikzpicture}


==> tables/forecasting_uni.tex <==
\begin{landscape}
\begin{table}[t]
\centering
\caption{Full results for univariate time-series forecasting using MSE and MAE as metrics. The reported scores for all comparison methods are taken from~\cite{ts2vec}. Note that for each method, pre-training and the downstream task are performed for each dataset individually. \mg{[Include LSTnet]}} \vspace{.5\baselineskip}
\label{tab:forecast_uni}
\begin{tabular}{lccccccccccccc}
\toprule
 & & \multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{TS2Vec \cite{ts2vec}} & \multicolumn{2}{c}{Informer \cite{ett_informer}} & \multicolumn{2}{c}{LogTrans \cite{logtrans}} & \multicolumn{2}{c}{N-BEATS \cite{nbeats}} & \multicolumn{2}{c}{TCN \cite{tcn}} \\
 \cmidrule(lr){3-4}  \cmidrule(lr){5-6}  \cmidrule(lr){7-8}  \cmidrule(lr){9-10}  \cmidrule(lr){11-12}  \cmidrule(lr){13-14}
Dataset & $H$ & MSE & MAE  & MSE & MAE  & MSE & MAE  & MSE & MAE  & MSE & MAE  & MSE & MAE \\
\midrule
& 24 & 0.049 & 0.1687 & \textbf{0.039} & \textbf{0.152} & 0.098 & 0.247 & 0.103 & 0.259 & 0.094 & 0.238 & 0.075 & 0.21 \\
& 48 & 0.0788 & 0.2149 & \textbf{0.062} & \textbf{0.191} & 0.158 & 0.319 & 0.167 & 0.328 & 0.21 & 0.367 & 0.227 & 0.402 \\
ETTh$_1$ & 168 & 0.1359 & 0.2867 & \textbf{0.134} & \textbf{0.282} & 0.183 & 0.346 & 0.207 & 0.375 & 0.232 & 0.391 & 0.316 & 0.493 \\
& 336 & 0.1579 & 0.3146 & \textbf{0.154} & \textbf{0.31} & 0.222 & 0.387 & 0.23 & 0.398 & 0.232 & 0.388 & 0.306 & 0.495 \\
& 720 & 0.2299 & 0.3869 & \textbf{0.163} & \textbf{0.327} & 0.269 & 0.435 & 0.273 & 0.463 & 0.322 & 0.49 & 0.39 & 0.557 \\
\midrule
& 24 & \textbf{0.0771} & \textbf{0.21} & 0.09 & 0.229 & 0.093 & 0.24 & 0.102 & 0.255 & 0.198 & 0.345 & 0.103 & 0.249 \\
& 48 & \textbf{0.1022} & \textbf{0.2468} & 0.124 & 0.273 & 0.155 & 0.314 & 0.169 & 0.348 & 0.234 & 0.386 & 0.142 & 0.29 \\
ETTh$_2$ & 168 & \textbf{0.1528} & \textbf{0.3089} & 0.208 & 0.36 & 0.232 & 0.389 & 0.246 & 0.422 & 0.331 & 0.453 & 0.227 & 0.376 \\
& 336 & \textbf{0.1832} & \textbf{0.3386} & 0.213 & 0.369 & 0.263 & 0.417 & 0.267 & 0.437 & 0.431 & 0.508 & 0.296 & 0.43 \\
& 720 & \textbf{0.2072} & \textbf{0.3679} & 0.214 & 0.374 & 0.277 & 0.431 & 0.303 & 0.493 & 0.437 & 0.517 & 0.325 & 0.463 \\
\midrule
& 24 & 0.0168 & 0.0979 & \textbf{0.015} & \textbf{0.092} & 0.03 & 0.137 & 0.065 & 0.202 & 0.054 & 0.184 & 0.041 & 0.157 \\
& 48 & 0.0306 & 0.1318 & \textbf{0.027} & \textbf{0.126} & 0.069 & 0.203 & 0.078 & 0.22 & 0.19 & 0.361 & 0.101 & 0.257 \\
ETTm$_1$ & 96 & 0.0521 & 0.1741 & \textbf{0.044} & \textbf{0.161} & 0.194 & 0.372 & 0.199 & 0.386 & 0.183 & 0.353 & 0.142 & 0.311 \\
& 288 & 0.1087 & 0.2565 & \textbf{0.103} & \textbf{0.246} & 0.401 & 0.554 & 0.411 & 0.572 & 0.186 & 0.362 & 0.318 & 0.472 \\
& 672 & 0.1623 & 0.3156 & \textbf{0.156} & \textbf{0.307} & 0.512 & 0.644 & 0.598 & 0.702 & 0.197 & 0.368 & 0.397 & 0.547 \\
\midrule
& 24 & 0.2723 & 0.3857 & 0.26 & 0.288 & \textbf{0.251} & \textbf{0.275} & 0.528 & 0.447 & 0.427 & 0.33 & 0.263 & 0.279 \\
& 48 & \textbf{0.3026} & 0.4024 & 0.319 & \textbf{0.324} & 0.346 & 0.339 & 0.409 & 0.414 & 0.551 & 0.392 & 0.373 & 0.344 \\
Electricity & 168 & \textbf{0.3374} & 0.4314 & 0.427 & \textbf{0.394} & 0.544 & 0.424 & 0.959 & 0.612 & 0.893 & 0.538 & 0.609 & 0.462 \\
& 336 & \textbf{0.36} & \textbf{0.4487} & 0.565 & 0.474 & 0.713 & 0.512 & 1.079 & 0.639 & 1.035 & 0.669 & 0.855 & 0.606 \\
& 720 & \textbf{0.3593} & \textbf{0.4533} & 0.861 & 0.643 & 1.182 & 0.806 & 1.001 & 0.714 & 1.548 & 0.881 & 1.263 & 0.858 \\
\midrule
Avg. & & \textbf{0.1688} & 0.2971 & 0.209 & \textbf{0.296} & 0.31 & 0.39 & 0.37 & 0.434 & 0.399 & 0.426 & 0.338 & 0.413 \\
\bottomrule
\end{tabular}
\end{table}
\end{landscape}
